Reduced etch lag and high aspect ratios by deep reactive ion etching (DRIE)

Deep reactive ion etching (DRIE) with the Bosch process is one of the key procedures used to manufacture micron-sized structures for MEMS and microfluidic applications in silicon and, hence, of increasing importance for miniaturization in biomedical research. While guaranteeing high aspect ratio structures and providing high design flexibility, the etching procedure suffers from reactive ion etching lag and often relies on complex oxide masks to enable deep etching. In this work, we introduce an optimized Bosch process that reduces the etch lag to below 1.5 %. Furthermore, we improved a three-step Bosch process, allowing the fabrication of structures with 6 micrometre thickness at depths up to 180 micrometre while maintaining their stability.

==> Sections/Aussortiert.tex <==
Etching is one of the most complex processes and can be roughly divided into wet and dry etching dependant on the used etchant. Wet etching often utilizes KOH and ... used for ... The main limitations of wet etching are its low selectivity (ratio of mask to silicon etching), the mask needs to be chemically resitant towards the etchant and isotropic etching. The isotropy can be counteracted with etching along the crystal-orientation of the silicon, thus only allowing designs with $\SI{45}{\degree}$ angles.
Dry etching is based on the ion bombardment from a plasma generated in the etch chamber. 

It is important to highlight that the dimensions on the chrome mask do not precisely match the dimensions transferred to the silicon wafer. Typically, $\SI{100}{\micro\meter}$ wide channels are $\SI{3}{\micro\meter}$ wider than on the mask. We experienced that this deviation increases linearly with the width of the channel. 

Sketch of the Bosch process parameters for a standard procedure (top) and the optimized process parameters (bottom). A gas flow of 10 sscm is always maintained to enable faster switching times (violet horizontal bar). (b) Optical microscopy images of diced silicon wafers to illustrate the improvement in RIE lag. (top) Trenches etched with the standard Bosch process, with $\SI{20}{\micro\meter}$ to $\SI{3}{\micro\meter}$ wide trenches reached a depths of $\SI{64}{\micro\meter}$ and $\SI{47}{\micro\meter}$, respectively, corresponding to an RIE lag of $\SI{27}{\percent}$. (bottom) Trenches etched with our optimized process, with (I) $\SI{20}{\micro\meter}$, (II) $\SI{15}{\micro\meter}$, (III) $\SI{10}{\micro\meter}$, and (IV) $\SI{5}{\micro\meter}$ width were etched $\SI{47.8}{} \pm \SI{0.7}{\micro\meter}$ deep into the silicon wafer with an etch angle $\alpha = \SI{91.5}{\degree}$. We managed to reduce the RIE lag with our new recipe such that the depth of the different tranches only vary within $\SI{1.9}{\micro\meter}$, corresponding to a RIE lag of below $\SI{1.5}{\percent}$. Scale bars corresponding to $\SI{25}{\micro\meter}$.
